Constructive reflectivity principles for regular theories

Classically, any structure for a signature $\Sigma$ may be completed to a model of a desired regular theory $T$ by means of the chase construction or small object argument. Moreover, this exhibits $\mathrm{Mod}(T)$ as weakly reflective in $\mathrm{Str}(\Sigma)$. We investigate this in the constructive setting. The basic construction is unproblematic; however, it is no longer a weak reflection. Indeed, we show that various reflectivity principles for models of regular theories are equivalent to choice principles in the ambient set theory. However, the embedding of a structure into its chase-completion still satisfies a conservativity property, which suffices for applications such as the completeness of regular logic with respect to Tarski (i.e. set) models. Unlike most constructive developments of predicate logic, we do not assume that equality between symbols in the signature is decidable. While in this setting, we also give a version of one classical lemma which is trivial over discrete signatures but more interesting here: the abstraction of constants in a proof to variables

==> non-discrete-macros.tex <==

% Sectioning commands

\makeatletter
\newcommand\myparagraph{\@startsection{paragraph}{4}{0pt}%
                                  {\medskipamount}%
                                  {-0pt}%
                                  {\normalfont\normalsize\bfseries}}
\makeatother

\opt{jsl}{
  \newcommand{\subtleparagraph}[1][]{\medskip \paragraph{#1}}
  % Note to JSL typesetters: we use \paragraph-level sectioning without an explicit heading, so we add a \medskip to make these visible.  If this violates ASL style too much, please remove "subtleparagraph" where no argument is given, and replace it with "paragraph" where an argument is given

  \newcommand{\case}[1]{\subtleparagraph{(#1)}}
}
\opt{arxiv}{
  \newcommand{\subtleparagraph}[1][]{\myparagraph{#1}}

  \newcommand{\case}[1]{\subtleparagraph{(#1)}}
}

% Title tweaking to include note

\makeatletter
\opt{arxiv}{

  % lightly tweaked from article.cls 
  \def\@maketitle{%
  \newpage
  \null
  \vskip 0.8em% orig 2em
  \begin{center}%
  \let \footnote \thanks
    {\LARGE \@title \par}%
    \vskip 1.2em% orig 1.5em
    {\large
      \lineskip .4em% orig .5em
      \begin{tabular}[t]{c}%
        \@author
      \end{tabular}\par}%
    \vskip 0.8em% orig 1em
    {\large \@date}%
%   \vskip 0.8em% ADDED
%    {\small \@titlenote}% ADDED
  \end{center}%
  \par
  \vskip 0.5em}% orig 1.5em 

  \newcommand{\titlenote}[1]{\gdef \@titlenote {#1}}
  \newcommand{\maketitlenote}[1]{%
    \begin{center}
    \small \@titlenote
    \end{center}
  }

  \newcommand{\arxiv}[1]{\href{https://arxiv.org/abs/#1}{arXiv:\thinspace\nolinkurl{#1}}}

  \newcommand{\doi}[1]{\href{https://dx.doi.org/#1}{\textsc{doi:}\thinspace\nolinkurl{#1}}}
}
\makeatother



% Diagram commands

%diagramas
%\input{xy}
%\usepackage[all]{xy}
%\newdir{ >}{{}*!/-5pt/@{>}}
%\newcommand{\comp}[2]{\ensuremath{\{ #1 \ |\ #2 \}}}
\input{diagxy}
\xyoption{curve}

\newbox\anglebox % large pullback angle
\setbox\anglebox=\hbox{\xy \POS(75,0)\ar@{-} (0,0) \ar@{-} (75,75)\endxy}
 \def\pbangle{\copy\anglebox}
\newbox\angleboxr % reverse large pullback angle
\setbox\angleboxr=\hbox{\xy \POS(0,0)\ar@{-} (0,75) \ar@{-} (75,0)\endxy}
 \def\pbangler{\copy\angleboxr}
\newbox\sanglebox % small pullback angle
\setbox\sanglebox=\hbox{\xy \POS(50,0)\ar@{-} (0,0) \ar@{-} (50,50)\endxy}
 \def\spbangle{\copy\sanglebox}
\newbox\sangleboxr % small reverse pullback angle
\setbox\sangleboxr=\hbox{\xy \POS(0,0)\ar@{-} (0,50) \ar@{-} (50,0)\endxy}
 \def\spbangler{\copy\sangleboxr}
\newbox\sangleboxf % small flipped pullback angle
\setbox\sangleboxf=\hbox{\xy \POS(50,50)\ar@{-} (50,0) \ar@{-} (0,50)\endxy}
 \def\spbanglef{\copy\sangleboxf}
\newbox\angleboxf % flipped pullback angle
\setbox\angleboxf=\hbox{\xy \POS(75,75)\ar@{-} (75,0) \ar@{-} (0,75)\endxy}
\def\pbanglef{\copy\angleboxf}
\newbox\sangleboxfr % small flipped reverse pullback angle
\setbox\sangleboxfr=\hbox{\xy \POS(0,50)\ar@{-} (50,50) \ar@{-} (0,0)\endxy}
 \def\spbanglefr{\copy\sangleboxfr}
\newbox\angleboxfr % small flipped reverse pullback angle
\setbox\angleboxfr=\hbox{\xy \POS(0,75)\ar@{-} (75,75) \ar@{-} (0,0)\endxy}
\def\pbanglefr{\copy\angleboxfr}




%%%%
%% MACROS
%%%%

%% Fonts for types of objects.
\newcommand{\cat}[1]{\ensuremath{\mathcal{#1}}} % for e.g. “C”, not names like “Set”
\newcommand{\catname}[1]{\ensuremath{\mathrm{#1}}}
\newcommand{\thry}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\alg}[1]{\ensuremath{\mathbf{#1}}}

%% Styled letters
\newcommand{\C}{\mathbf{C}}
\newcommand{\Diag}[1]{\thry{D}_{#1}}
\newcommand{\E}[1]{{\thry{E}_{#1}}}
\newcommand{\F}[1]{{\thry{F}_{#1}}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\nat}{\ensuremath{\mathbb{N}}}
\newcommand{\theory}{\thry{T}}
\newcommand{\R}{\mathcal{R}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}

\newcommand{\backE}[1]{{{}^E{#1}}}

\newcommand{\arity}[1]{n_{#1}}

% “vectors”/tuples
\newcommand{\tupleletter}[1]{\mathbf{#1}}

\renewcommand{\a}{\tupleletter{a}}
\renewcommand{\b}{\tupleletter{b}}
\newcommand{\cc}{\tupleletter{c}} % Can’t use “\c”, since that’s ç, needed in the bibliography. 
\newcommand{\dd}{\tupleletter{d}}
\newcommand{\s}{\tupleletter{s}}
\renewcommand{\t}{\tupleletter{t}}
\newcommand{\w}{\tupleletter{w}}
\newcommand{\x}{\tupleletter{x}}
\newcommand{\y}{\tupleletter{y}}
\newcommand{\z}{\tupleletter{z}}

\newcommand{\test}[1][]{%
\ifthenelse{\equal{#1}{}}{omitted}{given}%
}

%% Logical syntax
\newcommand{\proves}{\vdash}
\newcommand{\believes}{\vDash}
\newcommand{\fins}[1]{\exists {#1}\mathpunct .}
\newcommand{\Tm}[2][]{\ifthenelse{\equal{#2}{}}%
  {\mathrm{Tm}_{#1}}%
  {\mathrm{Tm}_{#1}(#2)}}
\opt{jsl}{\providecommand{\Form}{}} % arxiv version has \Form already from hyperref; so we need \renewcommand{\Form} below
\renewcommand{\Form}[2][]{\ifthenelse{\equal{#2}{}}%
  {\mathrm{Form}_{#1}}%
  {\mathrm{Form}_{#1}(#2)}}
\newcommand{\conj}{\bigwedge}
\newcommand{\FV}{FV}
\newcommand{\ltrue}{\top}
\newcommand{\lfalse}{\bot}

\newcommand{\Rel}{\mathrm{Rel}}
\newcommand{\Fun}{\mathrm{Fun}}

%% General categorical operations
\newcommand{\comp}{\cdot}
\newcommand{\name}[1]{\ulcorner #1 \urcorner}
\newcommand{\adjoint}{\dashv}
\newcommand{\orthog}{\pitchfork}
\DeclareMathOperator{\cod}{cod}
\DeclareMathOperator{\dom}{dom}

%% Category names
\newcommand{\Str}[1]{\ensuremath{\catname{Str}(#1)}}
\newcommand{\Mod}[1]{\ensuremath{\catname{Mod}(#1)}}
\newcommand{\Set}{\mathbf{Set}}

\newcommand{\arr}{\rightarrow}

\newcommand{\Br}[2]{\mathrm{Br}_{#1}(#2)}

%% Axiom names
% TODO: add xspace for these?
\newcommand{\PAx}{\ensuremath{\mathrm{PAx}}}
\newcommand{\AC}{\ensuremath{\mathrm{AC}}}
\newcommand{\coshep}{\ensuremath{\mathrm{CoSHEP}}}
\newcommand{\WISC}{\ensuremath{\mathrm{WISC}}}
\newcommand{\WIC}{\ensuremath{\mathrm{WIC}}}
\newcommand{\DC}{\ensuremath{\mathrm{DC}}}
\newcommand{\RDC}{\ensuremath{\mathrm{RDC}}}
\newcommand{\RRS}{\ensuremath{\mathrm{RRS}}}
\newcommand{\ZF}{\ensuremath{\mathrm{ZF}}}
\newcommand{\REA}{\ensuremath{\mathrm{REA}}}
\newcommand{\CZF}{\ensuremath{\mathrm{CZF}}}
\newcommand{\AMC}{\ensuremath{\mathrm{AMC}}}

%% Notation for the chase
\newcommand{\chase}[2][]{\ensuremath{\operatorname{Ch}_{#1}({#2})}}
\newcommand{\chasef}[1]{\ensuremath{\operatorname{Ch}_{#1}}}
\newcommand{\onestep}[2][]{\ensuremath{\mathrm{ex}_{#1}{(#2)}}}
\newcommand{\severalsteps}[2][]{\ensuremath{\mathrm{ex}^{#1}{(#2)}}}

\newcommand{\idx}{\ensuremath{\operatorname{idx}}}

\newcommand{\syntstr}[2]{\ensuremath{\langle \! \langle #1\mid    #2\rangle \! \rangle}}

%% Binders, delimiters
\newcommand{\pair}[1]{\ensuremath{\langle {#1} \rangle}}
\newcommand{\family}[2]{\langle #1 \rangle_{#2} }

\newcommand{\domain}[1]{|#1|}
\newcommand{\lscott}{[\![}
\newcommand{\rscott}{]\!]}
\newcommand{\sem}[1]{\ensuremath{\lscott  {#1} \rscott}}
\newcommand{\interp}[2][]{\sem{#2}^{#1}} % alias
\newcommand{\csem}[2]{\ensuremath{\lscott {#1} \mathbin{|} {#2} \rscott}} % withcontext
\newcommand{\cterm}[2]{\ensuremath{\{ {#1} \mathbin{|} {#2} \}}}

%\newcommand{\syntob}[2]{\ensuremath{[{#1} \mathbin{|} {#2}]}}

\newcommand{\syntob}[2]{\ensuremath{{#1} \ldotp {#2}}}
\newcommand{\fmlcxt}[2]{\syntob{#2}{#1}} % alias

%% Arrows, diagrams, and similar
% TODO: improve and consistentise these
\newcommand{\funktor}[3]{\ensuremath{\operatorname{#1} \! :\!  #2 \to<125> #3}}
\newcommand{\into}{\to/^{ (}->/}
\newcommand{\iso}{\cong}
\renewcommand{\equiv}{\simeq}
\newcommand{\surjto}{\to/->>/}
\newcommand{\Imp}{\Rightarrow}
\newcommand{\ImpliedBy}{\Leftarrow}
\newcommand{\Equiv}{\Leftrightarrow}
\DeclareMathSymbol{\exclamdown}{\mathord}{operators}{"BD} % May need to change depending on font encoding; see http://tex.stackexchange.com/a/103437/1635
\newcommand{\gnab}[1]{\exclamdown_{#1}}

\newcommand{\colim}{\varinjlim}

%% Draft annotations
\newcommand{\todo}[1]{\marginpar{\textcolor{red}{#1}}}
\newcommand{\handptodo}[1]{\marginpar{\textcolor{purple}{#1}}}
\newcommand{\htodo}[1]{\marginpar{\textcolor{blue}{#1}}}
\newcommand{\hkomment}[1]{\marginpar{\textcolor{green}{#1}}}
\newcommand{\placeholder}[1]{\textcolor{red}{#1}}
\newcommand{\hplaceholder}[1]{\textcolor{blue}{#1}}
\newcommand{\hfotnot}[1]{\footnote{\textcolor{blue}{#1}}}
%
\newcommand{\hbokm}{\hplaceholder{Jag \"{a}r h\"{a}r}}

